A Groupoid Picture of Elek Algebras

We describe a construction by G\'abor Elek, associating C*-algebras with uniformly recurrent subgroups, in the language of groupoid C*-algebras. This allows us to simplify several proofs in the original paper and fully characterise their nuclearity. We furthermore relate our groupoids to the dynamics of the group acting on its uniformly recurrent subgroup.

==> localPropertyA.tex <==
\section{A Converse Implication For Nuclearity}
\label{sec:locPropA}
As a benefit of our description of $\Csred(Z)$ 
as the reduced algebra of a groupoid,
we are able to add the converse implication 
to Corollary \ref{cor:locPropANuclear},
and show that $\Csred(Z)$ is nuclear
if and only if the associated Schreier graphs
$\Schreier(H)$ have local property A
for any $H\in Z$.

We first give a converse 
to Proposition \ref{prop:locPropANuclear}.

\begin{proposition}\label{Prop:PushBackA}
  Suppose $\G$ is (topologically) amenable. 
  Then $\Schreier(H)$ has local property $A$.
\end{proposition}
\begin{proof}
  By an equivalent characterisation of amenability \cite[Prop 2.2.13]{AmenableGrpd}, 
  we may assume that there is a sequence $f_n\in \C_c(\G)$, 
  such that
  \begin{align*}
    \sum\limits_{(u,\gamma)\in \G^u} |f_n(u,\gamma)|^2 &\xrightarrow{n\to\infty} 1 
    \text{ uniformly on compact subsets of $\G^0$ as a function of $u$}\\
    \text{and} 
    \sum\limits_{h\in \G^{r(g)}} |f_n(g^{-1}h) - f_n(h)|^2 &\xrightarrow{n\to\infty} 0 
    \text{ uniformly on compact subsets of $\G$ as a function of $g$.}
  \end{align*}
  To obtain local maps $\rho^n_x$ 
  as in the definition of local property A,
  we first, for any $\eps>0$,
  approximate $f_n$ by (uniformly) locally constant functions $f_{n,\eps}\in \C_c(\G)$
  such that $\|f_n - f_{n,\eps}\|_\infty < \eps$, 
  choosing $f_{n,\eps}$ to be zero on the largest possible ball 
  centred at $\centralstar$.

  We next construct a sequence $\eps_n \searrow 0$, 
  such that $f_{n,\eps_n}$ satisfies the convergence properties above:
  As for fixed $n$ there is $T_n\in N$ 
  such that both $f_n$ and $f_{n,\eps}$
  for every $\eps>0$ 
  vanish on the $2^{-T_n}$-ball of $\centralstar$ 
  we may restrict summation to arrows
  described by group elements $\gamma$
  with length $l(\gamma)$ at most $T_n$,
  such that the respective sums become finite
  with less than $(|Q| + 1)^{T_n}$ terms.
  %\begin{align*}
  %  \sum\limits_{(u,\gamma)\in \G^u} |f_n(u,\gamma)|^2 
  %  = \sum\limits_{\substack{(u,\gamma)\in \G^u,\\ l(\gamma)<T_n}} |f_n(u,\gamma)|^2
  %  \quad\text{and}\quad
  %  \sum\limits_{(u,\gamma)\in \G^u} |f_{n,\eps}(u,\gamma)|^2 
  %  = \sum\limits_{(u,\gamma)\in \G^u, l(\gamma)<T_n} |f_{n,\eps}(u,\gamma)|^2.
  %\end{align*}
  Therefore,
  \begin{align*}
    \left|\sum\limits_{(u,\gamma)\in \G^u} 
      |f_n(u,\gamma)|^2 - \sum\limits_{(u,\gamma)\in \G^u} 
      |f_{n,\eps}(u,\gamma)|^2\right|
      &\leq \sum\limits_{\substack{(u,\gamma)\in \G^u,\\l(\gamma)\leq T_n}}
      (|f_n(u,\gamma)| + \eps)^2 - |f_{n}(u,\gamma)|^2\\
    &\leq (|Q|+1)^{T_n}(2\|f_n\|_\infty + \eps)\eps 
    \xrightarrow{\eps\to 0} 0,
  \intertext{
  with the convergence uniformly in $u \in \G^0$.
  Likewise, we calculate
  }
    \sum\limits_{h\in \G^{r(g)}} |f_{n,\eps}(g^{-1}h) - f_{n,\eps}(h)|^2
    &\leq \sum\limits_{h\in \G^{r(g)}, l(\gamma)\leq T_n} (|f_{n}(g^{-1}h) - f_{n}(h)|+2\eps)^2\\
    &\leq (4\eps^2 + 8\eps \|f_n\|_\infty)(|Q|+1)^{T_n} 
    + \sum\limits_{h\in \G^{r(g)}} |f_{n}(g^{-1}h) - f_{n}(h)|^2 
    \\
    &\xrightarrow{\eps \to 0}
    \sum\limits_{h\in \G^{r(g)}} |f_{n}(g^{-1}h) - f_{n}(h)|^2,
  \intertext{
  with the convergence uniformly in $g\in \G$.
  Picking $\eps_n\to 0$ such that 
  }
  1/n &\geq
  (|Q|+1)^{T_n}(2\|f_n\|_\infty + \eps_n)\eps_n 
  \\
  \text{and}\qquad
  1/n &\geq
  (4\eps_n^2 + 8\eps_n \|f_n\|_\infty)(|Q|+1)^{T_n} 
  \end{align*}
  does the trick.
  To such $f_{n,\eps_n}$ 
  we may assign $\rho^{n} \colon \Gamma/H \rightarrow l^2(\Gamma/H)$ 
  by $\rho^{n}_x(\gamma x) = f_{n,\eps_n}([[x]], \gamma)$.

  Picking $S_{n}$ such that $f_{n,\eps_n}$ is  constant on any $2^{-S_{n}}$-ball,
  we see that $\rho^{n}_x$ is supported on $B_{S_{n}}(x)$, 
  since $f_{n,\eps_n}$ vanishes on the $2^{-S_{n}}$-neighbourhood 
  of $\centralstar$.
  Similarly,
  $\rho^{n}_x(\gamma x) = \rho^{n}_y(\gamma y)$ 
  for $l(\gamma)\leq S_{n}$ if the $S_{n}$-balls around $x$ and $y$ are isomorphic, 
  as $([[x]],\gamma)$ and $([[y]], \gamma)$ are $2^{-S_{n}}$-close in that case
  and we conclude that $\rho_n$ is local
  of width $S_n$.

  Furthermore, we compute that
  \begin{align*}
    \|\rho^{n}_{\gamma H}\|_2^2 
    &= \sum\limits_{\gamma'H\in \G/H} |\rho^{n}_{\gamma H}(\gamma'H)|^2
    = \sum\limits_{([[\gamma H]],\gamma')\in \G^u} |f_{n,\eps_n}([[\gamma H]],\gamma')|^2 
    \xrightarrow{n\to\infty} 1
    \intertext{converges uniformly on $\G^0$. Likewise,}
    \|\rho^{n}_{\gamma H} - \rho^{n}_{\gamma'H}\|_2^2
    &= \sum \limits_{\eta H \in \Gamma/H} |\rho^{n}_{\gamma H}(\eta H) - \rho^{n}_{\gamma'H}(\eta H)|^2\\
    &= \sum\limits_{\eta H \in \Gamma/H} | f_{n,\eps_n}(\gamma[[H]], \eta\gamma^{-1}) - f_{n,\eps_n}(\gamma'[[H]], \eta(\gamma')^{-1})|^2\\
    &= \sum\limits_{\eta H \in \Gamma/H} | f_{n,\eps_n}\left((\gamma[[H]], \gamma'\gamma^{-1})(\gamma'[[H]], \eta(\gamma')^{-1})\right) - f_{n,\eps_n}(\gamma'[[H]], \eta(\gamma')^{-1})|^2\\
    &= \sum\limits_{\eta H \in \Gamma/H} | f_{n,\eps_n}\left((\gamma'[[H]], \gamma(\gamma')^{-1})^{-1}(\gamma'[[H]], \eta(\gamma')^{-1})\right) - f_{n,\eps_n}(\gamma'[[H]], \eta(\gamma')^{-1})|^2\\
    &= \sum\limits_{h \in \G^{\gamma'[[H]]}} | f_{n,\eps_n}\left((\gamma[[H]], \gamma'\gamma^{-1})h\right) - f_{n,\eps_n}(h)|^2
    \xrightarrow {n\to\infty} 0
  \end{align*}
  converges uniformly for $(\gamma'[[H]], \gamma(\gamma')^{-1})$ in compact subsets of $\G$. 
  In particular, the convergence is uniform, 
  when the pair $(\gamma, \gamma')$ is taken from a subset with bounded difference, 
  that is, if there is $N>0$ such that
  $l(\gamma(\gamma')^{-1}) < N$.
  More importantly, 
  this means that
  for any $N\in \N$ 
  we may choose $n_0\in \N$, 
  such that $\|\rho^n_{\gamma H} - \rho^n_{\gamma'H}\|_2^2\leq 1/N$, 
  whenever $d_{\Schreier(H)}(\gamma H, \gamma'H) \leq N$ 
  and $n\geq n_0$.
  The analogous statement holds after replacing $\rho^n_x$
  with the normed function $\hat\rho^n_x = \rho^n_x/\|\rho^n_x\|_2$,
  since the convergences indicated in the following estimate are uniform:
  \begin{align*}
    \|\hat\rho^n_{\gamma H} - \hat \rho^n_{\gamma' H}\|_2
    &\leq \underbrace{\frac{1}{\|\rho^n_{\gamma H}\|_2}}_{\to 1} 
    \left( 
      \|\rho^n_{\gamma H} - \rho^n_{\gamma'H}\|_2 
      + \underbrace{ \left| \|\rho^n_{\gamma H}\|_2 - \|\rho^n_{\gamma' H}\|_2\right|}
      _{\to 0}
    \right)
  \end{align*}
  Then, after relabelling, 
  $\hat\rho^n$ witnesses local property A of $\Schreier(H)$.
\end{proof}

For \etale{} groupoids there is a clear relation
between amenability and nuclearity of their reduced \Csalgebra{}s,
which directly translates to our case:
\begin{corollary}
  Let $Z$ be a uniformly recurrent subgroup and $H\in Z$.
  The graph $\Schreier(H)$ has local property A
  if and only if
  the \Csalgebra{} $\Csr(Z)$ is nuclear.
\end{corollary}
\begin{proof}
  As $\G$ is \etale, 
  $\Csr(\G)$ is nuclear if and only if 
  $\G$ is (topologically) amenable by \cite[Corollary 6.2.14]{AmenableGrpd}.
  Therefore, 
  Proposition \ref{Prop:PushBackA} gives the converse implication 
  to Corollary \ref{Cor:ANuc}.
\end{proof}

\begin{remark}
  A minimal \emph{amenable} second countable \etale{} groupoid 
  has simple reduced \Csalgebra, 
  if and only if it is topologically principal.
  Hence, if the Schreier graphs of $Z$ have local property $A$, 
  then $\Csr(Z)$ is simple if and only if $Z$ is generic.

  More generally, 
  $\Csr(Z)$ is simple 
  for arbitrary URS $Z$,
  if and only if $\Csr(\G)$ has the \emph{intersection property} 
  relative to $\C_0(\G^0)$,
  meaning that every (nontrivial) ideal of $\Csr(\G)$
  intersects $\C_0(\G^0)$ nontrivially.
\end{remark}


==> reproduction.tex <==
\section{Simplicity and Nuclearity}
\label{sec:reproduction}

We employ our description of the Elek algebras as groupoid algebras
to give simplified proofs of Elek's characterisations,
explaining why they arise, at least in the language of groupoids.
\begin{proposition}\label{prop:generic-principal}
	If $Z$ is generic, then $\G$ is principal.
\end{proposition}
\begin{proof}
  Suppose $\G$ is not principal.
  Then there is a unit $x=([x_0]_0, [x_1]_1, \ldots)$
  and an arrow in the isotropy $\G_x^x$ that is not a unit.
  Therefore there is a group element $\gamma \in \Gamma$ 
  such that $x = \gamma.x$ but $(x, e) \neq (x, \gamma)$.
  Especially $\gamma.x_N \neq x_N$ for large N, 
  while $B_{N-l(\gamma)}(S,x_N) \rlisom B_{N-l(\gamma)}(S,\gamma.x_N)$ 
  and $d(x_N, \gamma.x_N)\leq  l(\gamma)$.
  By \cite[Proposition 2.3]{Elek_URS}, $Z$ is not generic.
\end{proof}

\begin{corollary}
	If $Z$ is generic, then $\Csr(Z)$ is simple.
\end{corollary}
This reproduces \cite[Theorem 7]{Elek_URS}.
\begin{proof}
	By Proposition \ref{prop:generic-principal}, 
    $\G$ is a minimal principal \etale{} groupoid,
    and every such groupoid has a simple reduced \Csalgebra{}
    by \cite[Proposition 4.3.7]{SimsNotes}.
\end{proof}

\begin{proposition}
  \label{prop:locPropANuclear}
	If $Z$ is a uniformly recurrent subgroup 
    such that $\Schreier(H)$ has local property A for any $H\in Z$, 
	then $\G$ is (topologically) amenable.
\end{proposition}
\begin{proof}
	Let $\G$ be constructed from $H\in Z$ 
    and let $\rho^n\colon \Gamma/H \rightarrow l^2(\Gamma/H)$ 
    implement local property $A$ of $S_\Gamma^Q(H)$.
	Let $S_n$ describe the locality of $\rho^n$ 
    as in Section \ref{sec:introduction}.
    Let $x_{S_n}$ denote any element of the equivalence class of $E_{S_n}$
    forming the $S_n$-component of $x$
    and define $f_n\in \C_c(\G)$ by $f_n(x, \gamma) = \rho^n_{x_{S_n}}(\gamma.x_{S_n})$.
    This is independent of the choice of $x_{S_n}$,
    as $\rho^n$ are locally defined and of width at most $S_n$, 
	continuous as it is constant on $2^{-S_n}$-balls and compactly supported,
    as it vanishes on the $2^{-S_n}$-ball of $\centralstar$.
	For any unit $u\in \G^0$ we have
	\begin{align*}
		\sum\limits_{(u, \gamma) \in \G^u} |f_n(u,\gamma)|^2
		&= \sum\limits_{y \in B_{S_n}(u_{S_n})} |\rho^n_{u_{S_n}}(y)|^2
		= \|\rho^n_{u_{S_n}}\|_2^2 = 1,
	\intertext{
	using that $\rho^n_{x}$ is supported in the $S_n$-ball centred at $u_{x}$.
	Furthermore, we calculate
	}
		f_n \ast f_n^\ast(x,\gamma)
		&= \sum\limits_{(\gamma.x, \gamma') \in \G^{\gamma.x}}
        f_n((x,\gamma)(\gamma.x, \gamma')) \overline{f_n}(\gamma.x, \gamma'),
	\intertext{ 
      where we may restrict to $l(\gamma')\leq S_n$, 
      as $f_n(\gamma.x, \gamma')$ vanishes otherwise,
    }
 		&= \sum\limits_{(\gamma.x, \gamma') \in \G^{\gamma.x}, l(\gamma')\leq S_n}
        \rho^n_{x_{S_n + l(\gamma)}}(\gamma'\gamma x_{S_n + l(\gamma)}) 
			\overline{\rho^n_{\gamma x_{S_n + l(\gamma)}}}(\gamma'\gamma x_{S_n + l(\gamma)})\\
		&= \sum\limits_{z \in B_{S_n}(\gamma x_{S_n + l(\gamma)})}
        \rho^n_{x_{S_n + l(\gamma)}}(z) 
			\overline{\rho^n_{\gamma x_{S_n + l(\gamma)}}}(z)
		= \langle \rho^n_{x_{S_n + l(\gamma)}}, \rho^n_{\gamma x_{S_n + l(\gamma)}}\rangle,
	\end{align*}
	using again the assumptions on the support 
    of $\rho^n_{\gamma x_{S_n + l(\gamma)}}$.
	However, for fixed $u,v\in \Gamma/H$ we have
	\[
		\left| 1- \langle \rho^n_u, \rho^n_v\rangle\right| 
		= \left| \langle \rho^n_u - \rho^n_v, \rho^n_v\rangle \right|
		\leq \|\rho^n_u - \rho^n_v\|_2 \cdot \|\rho^n_v\|_2 
        \overset{(\dag)}\leq 1/n \cdot 1 
        \xrightarrow{n\to\infty} 0,
	\]
	where the estimate $(\dag)$ holds for large $n$ such that $d(u,v)\leq n$.
	But as $l(\gamma)$ is bounded on compact sets, 
    the same estimate may be used uniformly on any compact set for sufficiently large $n$,
	so that $f_n\ast f_n^\ast$ converges to one uniformly on compact subsets.
    Those functions witness the (topological) amenability of $\G$
    as in the original definition \cite[page 92]{Renault_GroupoidApproach}.
\end{proof}

%end of reproducing results
%beginning of adding converse implication

As a benefit of our description of $\Csred(Z)$ 
as the reduced algebra of a groupoid,
we are able to add the converse implication 
to Corollary \ref{cor:locPropANuclear},
and show that $\Csred(Z)$ is nuclear
if and only if the associated Schreier graphs
$\Schreier(H)$ have local property A
for any $H\in Z$.

We first give a converse 
to Proposition \ref{prop:locPropANuclear}.

\begin{proposition}\label{Prop:PushBackA}
  Suppose $\G$ is (topologically) amenable. 
  Then $\Schreier(H)$ has local property $A$.
\end{proposition}
\begin{proof}
  By an equivalent characterisation of amenability \cite[Prop 2.2.13]{AmenableGrpd}, 
  we may assume that there is a sequence $f_n\in \C_c(\G)$, 
  such that
  \begin{align*}
    \sum\limits_{(u,\gamma)\in \G^u} |f_n(u,\gamma)|^2 &\xrightarrow{n\to\infty} 1 
    \text{ uniformly on compact subsets of $\G^0$ as a function of $u$}\\
    \text{and} 
    \sum\limits_{h\in \G^{r(g)}} |f_n(g^{-1}h) - f_n(h)|^2 &\xrightarrow{n\to\infty} 0 
    \text{ uniformly on compact subsets of $\G$ as a function of $g$.}
  \end{align*}
  To obtain local maps $\rho^n_x$ 
  as in the definition of local property A,
  we first, for any $\eps>0$,
  approximate $f_n$ by (uniformly) locally constant functions $f_{n,\eps}\in \C_c(\G)$
  such that $\|f_n - f_{n,\eps}\|_\infty < \eps$, 
  choosing $f_{n,\eps}$ to be zero on the largest possible ball 
  centred at $\centralstar$.

  We next construct a sequence $\eps_n \searrow 0$, 
  such that $f_{n,\eps_n}$ satisfies the convergence properties above:
  As for fixed $n$ there is $T_n\in N$ 
  such that both $f_n$ and $f_{n,\eps}$
  for every $\eps>0$ 
  vanish on the $2^{-T_n}$-ball of $\centralstar$ 
  we may restrict summation to arrows
  described by group elements $\gamma$
  with length $l(\gamma)$ at most $T_n$,
  such that the respective sums become finite
  with less than $(|Q| + 1)^{T_n}$ terms.
  %\begin{align*}
  %  \sum\limits_{(u,\gamma)\in \G^u} |f_n(u,\gamma)|^2 
  %  = \sum\limits_{\substack{(u,\gamma)\in \G^u,\\ l(\gamma)<T_n}} |f_n(u,\gamma)|^2
  %  \quad\text{and}\quad
  %  \sum\limits_{(u,\gamma)\in \G^u} |f_{n,\eps}(u,\gamma)|^2 
  %  = \sum\limits_{(u,\gamma)\in \G^u, l(\gamma)<T_n} |f_{n,\eps}(u,\gamma)|^2.
  %\end{align*}
  Therefore,
  \begin{align*}
    \left|\sum\limits_{(u,\gamma)\in \G^u} 
      |f_n(u,\gamma)|^2 - \sum\limits_{(u,\gamma)\in \G^u} 
      |f_{n,\eps}(u,\gamma)|^2\right|
      &\leq \sum\limits_{\substack{(u,\gamma)\in \G^u,\\l(\gamma)\leq T_n}}
      (|f_n(u,\gamma)| + \eps)^2 - |f_{n}(u,\gamma)|^2\\
    &\leq (|Q|+1)^{T_n}(2\|f_n\|_\infty + \eps)\eps 
    \xrightarrow{\eps\to 0} 0,
  \intertext{
  with the convergence uniformly in $u \in \G^0$.
  Likewise, we calculate
  }
    \sum\limits_{h\in \G^{r(g)}} |f_{n,\eps}(g^{-1}h) - f_{n,\eps}(h)|^2
    &\leq \sum\limits_{h\in \G^{r(g)}, l(\gamma)\leq T_n} (|f_{n}(g^{-1}h) - f_{n}(h)|+2\eps)^2\\
    &\leq (4\eps^2 + 8\eps \|f_n\|_\infty)(|Q|+1)^{T_n} 
    + \sum\limits_{h\in \G^{r(g)}} |f_{n}(g^{-1}h) - f_{n}(h)|^2 
    \\
    &\xrightarrow{\eps \to 0}
    \sum\limits_{h\in \G^{r(g)}} |f_{n}(g^{-1}h) - f_{n}(h)|^2,
  \intertext{
  with the convergence uniformly in $g\in \G$.
  Picking $\eps_n\to 0$ such that 
  }
  1/n &\geq
  (|Q|+1)^{T_n}(2\|f_n\|_\infty + \eps_n)\eps_n 
  \\
  \text{and}\qquad
  1/n &\geq
  (4\eps_n^2 + 8\eps_n \|f_n\|_\infty)(|Q|+1)^{T_n} 
  \end{align*}
  does the trick.
  To such $f_{n,\eps_n}$ 
  we may assign $\rho^{n} \colon \Gamma/H \rightarrow l^2(\Gamma/H)$ 
  by $\rho^{n}_x(\gamma x) = f_{n,\eps_n}([[x]], \gamma)$.

  Picking $S_{n}$ such that $f_{n,\eps_n}$ is  constant on any $2^{-S_{n}}$-ball,
  we see that $\rho^{n}_x$ is supported on $B_{S_{n}}(x)$, 
  since $f_{n,\eps_n}$ vanishes on the $2^{-S_{n}}$-neighbourhood 
  of $\centralstar$.
  Similarly,
  $\rho^{n}_x(\gamma x) = \rho^{n}_y(\gamma y)$ 
  for $l(\gamma)\leq S_{n}$ if the $S_{n}$-balls around $x$ and $y$ are isomorphic, 
  as $([[x]],\gamma)$ and $([[y]], \gamma)$ are $2^{-S_{n}}$-close in that case
  and we conclude that $\rho_n$ is local
  of width $S_n$.

  Furthermore, we compute that
  \begin{align*}
    \|\rho^{n}_{\gamma H}\|_2^2 
    &= \sum\limits_{\gamma'H\in \G/H} |\rho^{n}_{\gamma H}(\gamma'H)|^2
    = \sum\limits_{([[\gamma H]],\gamma')\in \G^u} |f_{n,\eps_n}([[\gamma H]],\gamma')|^2 
    \xrightarrow{n\to\infty} 1
    \intertext{converges uniformly on $\G^0$. Likewise,}
    \|\rho^{n}_{\gamma H} - \rho^{n}_{\gamma'H}\|_2^2
    &= \sum \limits_{\eta H \in \Gamma/H} |\rho^{n}_{\gamma H}(\eta H) - \rho^{n}_{\gamma'H}(\eta H)|^2\\
    &= \sum\limits_{\eta H \in \Gamma/H} | f_{n,\eps_n}(\gamma[[H]], \eta\gamma^{-1}) - f_{n,\eps_n}(\gamma'[[H]], \eta(\gamma')^{-1})|^2\\
    &= \sum\limits_{\eta H \in \Gamma/H} | f_{n,\eps_n}\left((\gamma[[H]], \gamma'\gamma^{-1})(\gamma'[[H]], \eta(\gamma')^{-1})\right) - f_{n,\eps_n}(\gamma'[[H]], \eta(\gamma')^{-1})|^2\\
    &= \sum\limits_{\eta H \in \Gamma/H} | f_{n,\eps_n}\left((\gamma'[[H]], \gamma(\gamma')^{-1})^{-1}(\gamma'[[H]], \eta(\gamma')^{-1})\right) - f_{n,\eps_n}(\gamma'[[H]], \eta(\gamma')^{-1})|^2\\
    &= \sum\limits_{h \in \G^{\gamma'[[H]]}} | f_{n,\eps_n}\left((\gamma[[H]], \gamma'\gamma^{-1})h\right) - f_{n,\eps_n}(h)|^2
    \xrightarrow {n\to\infty} 0
  \end{align*}
  converges uniformly for $(\gamma'[[H]], \gamma(\gamma')^{-1})$ in compact subsets of $\G$. 
  In particular, the convergence is uniform, 
  when the pair $(\gamma, \gamma')$ is taken from a subset with bounded difference, 
  that is, if there is $N>0$ such that
  $l(\gamma(\gamma')^{-1}) < N$.
  More importantly, 
  this means that
  for any $N\in \N$ 
  we may choose $n_0\in \N$, 
  such that $\|\rho^n_{\gamma H} - \rho^n_{\gamma'H}\|_2^2\leq 1/N$, 
  whenever $d_{\Schreier(H)}(\gamma H, \gamma'H) \leq N$ 
  and $n\geq n_0$.
  The analogous statement holds after replacing $\rho^n_x$
  with the normed function $\hat\rho^n_x = \rho^n_x/\|\rho^n_x\|_2$,
  since the convergences indicated in the following estimate are uniform:
  \begin{align*}
    \|\hat\rho^n_{\gamma H} - \hat \rho^n_{\gamma' H}\|_2
    &\leq \underbrace{\frac{1}{\|\rho^n_{\gamma H}\|_2}}_{\to 1} 
    \left( 
      \|\rho^n_{\gamma H} - \rho^n_{\gamma'H}\|_2 
      + \underbrace{ \left| \|\rho^n_{\gamma H}\|_2 - \|\rho^n_{\gamma' H}\|_2\right|}
      _{\to 0}
    \right)
  \end{align*}
  Then, after relabelling, 
  $\hat\rho^n$ witnesses local property A of $\Schreier(H)$.
\end{proof}

\todocomment{streamline/fuse corollaries}
For \etale{} groupoids there is a clear relation
between amenability and nuclearity of their reduced \Csalgebra{}s,
which directly translates to our case:

\begin{corollary}\label{Cor:ANuc}
  \label{cor:locPropANuclear}
	If $Z$ is a uniformly recurrent subgroup 
    such that $\Schreier(H)$ has local property A for any $H\in Z$,
	then $\Csr(Z)$ is nuclear.
\end{corollary}
This reproduces \cite[Theorem 8]{Elek_URS}.
\begin{proof}
	As $\G$ is topologically amenable, 
    it is measurewise amenable and therefore $\Csr(\G)$ is nuclear.
	Compare for example \cite[Section 2]{Sims_AmenableFell} 
    for a brief overview of groupoid amenability.
\end{proof}

\begin{corollary}
  Let $Z$ be a uniformly recurrent subgroup and $H\in Z$.
  The graph $\Schreier(H)$ has local property A
  if and only if
  the \Csalgebra{} $\Csr(Z)$ is nuclear.
\end{corollary}
\begin{proof}
  As $\G$ is \etale, 
  $\Csr(\G)$ is nuclear if and only if 
  $\G$ is (topologically) amenable by \cite[Corollary 6.2.14]{AmenableGrpd}.
  Therefore, 
  Proposition \ref{Prop:PushBackA} gives the converse implication 
  to Corollary \ref{Cor:ANuc}.
\end{proof}

\begin{remark}
  A minimal \emph{amenable} second countable \etale{} groupoid 
  has simple reduced \Csalgebra, 
  if and only if it is topologically principal.
  Hence, if the Schreier graphs of $Z$ have local property $A$, 
  then $\Csr(Z)$ is simple if and only if $Z$ is generic.

  More generally, 
  $\Csr(Z)$ is simple 
  for arbitrary URS $Z$,
  if and only if $\Csr(\G)$ has the \emph{intersection property} 
  relative to $\C_0(\G^0)$,
  meaning that every (nontrivial) ideal of $\Csr(\G)$
  intersects $\C_0(\G^0)$ nontrivially.
\end{remark}

